A Fast-Convergence Routing of the Hot-Potato

Interactions between the intra- and inter-domain routing protocols received little attention despite playing an important role in forwarding transit traffic. More precisely, by default, IGP distances are taken into account by BGP to select the closest exit gateway for the transit traffic (hot-potato routing). Upon an IGP update, the new best gateway may change and should be updated through the (full) re-convergence of BGP, causing superfluous BGP processing and updates in many cases. We propose OPTIC (Optimal Protection Technique for Inter-intra domain Convergence), an efficient way to assemble both protocols without losing the hot-potato property. OPTIC pre-computes sets of gateways (BGP next-hops) shared by groups of prefixes. Such sets are guaranteed to contain the post-convergence gateway after any single IGP event for the grouped prefixes. The new optimal exits can be found through a single walk-through of each set, allowing the transit traffic to benefit from optimal BGP routes almost as soon as the IGP converges. Compared to vanilla BGP, OPTIC's structures allow it to consider a reduced number of entries: this number can be reduced by 99\% for stub networks. The update of OPTIC's structures, which is not required as long as border routers remain at least bi-connected, scales linearly in time with its number of groups.

==> ack.tex <==
This work was partially supported by the French National Research Agency (ANR) project Nano-Net under contract ANR-18-CE25-0003.

==> analysis.tex <==
%!TEX spellcheck = en_US
%!TEX root = ../info21.tex

We saw previously that the possible limitation of our solution is the number of 1-OP sets that a router has to manage.

In this section, we analyze the number of unique 1-OP sets depending on the number $B$ of gateways that learn new prefixes and on the policy spreading $ps$. Assuming each gateway learns every prefix with a weight chosen uniformly at random, we compute the average number $|{\opsets}_{B,ps}|$ of distinct 1-OP sets.
From this simple case, we deduce in the next section the feasibility of our solution in realistic scenarios.



From a global point of view, $|{\opsets}_{B,ps}|$ is the sum of distinct 1-OP sets of different sizes. We observe that 1-OP sets for different prefixes can be equal. For a given size $n \geq 2$, 1-OP sets of size $n$ are equiprobable, so let us denote $\P_{B, ps, P, n}$ the probability that at least one prefix, among all the $P$ prefixes, is associated with a given 1-OP set. Since there are $\binom{B}{n}$ such possible sets of size $n$, we have
\[
|{\opsets}_{B,ps}| = \sum_{n=2}^{B} \binom{B}{n} \P_{B, ps, P, n}.
\]

%First we need to compute the number of prefixes having 1-OP sets of size $n$.
For a given prefix, let $p_n$ be the probability that the size of its 1-OP set is $n$. Then, the number of prefixes associated with 1-OP sets of size $n$ is $p_nP$ on average. Thus, the probability that a given 1-OP set of size $n$ is not associated with any prefix is $\left(1-\binom{B}{n}^{-1}\right)^{p_nP}$. Hence, the probability that a given 1 OP set is associated with at least one prefix is

\[
\P_{B, ps, P, n} = 1-\left(1-\binom{B}{n}^{-1}\right)^{p_nP}.
\]

One can deduce two properties from those formulas. First, the number of distinct 1 OP sets of size $n$ is bounded by $\binom{B}{n}$, so the contribution of the cases $n = 1, 2$ in the sum is limited. Second, it is also bounded by $p_nP$, the average number of 1-OP sets of size $n$. We expect only a few prefixes with large 1-OP sets, so again the contribution of large $n$ in the sum is very limited. We will soon see that the vast majority of 1-OP sets are of size $n = 3$ as they occur with non-negligible probability and the number of such possible sets is too high to expect a lot of prefixes with the same 1-OP sets.

We now compute the probability $p_n$ for a given prefix to have a 1-OP set of size $n$.
Recall that we assumed each prefix is learned by all the gateways, and the weight associated with each gateway is chosen uniformly at random. The size of the 1-OP set for a given prefix is the number of gateways that learn this prefix with the minimum weight. However, if there is only one gateway with minimum weight, the 1-OP set also includes the gateways with the second minimum weight.

 The probability that $n$ given gateways have a given weight $i$ and the others have a weight greater than $i$ is ${1/ps^n(1-i/ps)^{B-n}}$, and that event can occur $\binom{B}{n}$ times. By summing that probability for all possible weigh $i$, we have that the probability that exactly $n$ gateways have the minimal weight is
\[
\sum\limits_{i=1}^{ps}
\binom{B}{n}\frac{1}{ps^{n}}\left(1-\frac{i}{ps}\right)^{B-n}.
\]
Similarly, the probability that $n-1$ gateways have weight $i$, one gateway has a smaller weight and the other gateways have greater weights is $\frac{1}{ps^{n-1}}\frac{i-1}{ps}\left(1-\frac{i}{ps}\right)^{B-n}$, and this event occurs $B\binom{B-1}{n-1}$ times. Summing up all the cases, we have:

\[
p_n = \sum\limits_{i=1}^{ps}
\frac{1}{ps^{n}}\left(1-\frac{i}{ps}\right)^{B-n}
\left(
(i-1)B\binom{B-1}{n-1} + \binom{B}{n}
\right)
\]

Here, the probability for a prefix to have a 1 OP set of size $n=3$ is relatively high. For instance, with $P=800,000$ and $B=ps=100$, we have $p_3\approx 0.267$, which gives 118,618 distinct 1-OP sets of size 3 in average.
If we apply our optimization, when a single gateway has the minimum weight, then the 1-OP set is of size 2, not matter how many gateways have the second minimum weight. Thus, the probability $p_n^\mathit{optim}$ of having a 1-OP set of size $n\geq 3$ is only the probability that exactly $n$ gateways have the minimum weight. The case $n=2$ is obtained by summing the probability that one or two gateways have the minimum weight:

\[
p_n^\mathit{optim}=\left\{
\begin{array}{ll}
\sum\limits_{i=1}^{ps}\frac{B}{ps}\left(1-\frac{i}{ps}\right)^{B-1} + \binom{B}{2}\frac{1}{ps^{2}}\left(1-\frac{i}{ps}\right)^{B-2}&\,\text{if }n=2\\
\sum\limits_{i=1}^{ps}\binom{B}{n}\frac{1}{ps^{n}}\left(1-\frac{i}{ps}\right)^{B-n} &\,\text{if }n\geq3
\end{array}
\right.
\]

As a comparison, with $P=800,000$ and $B=ps=100$, we have $p_3^\mathit{optim}\approx 0.097$, which gives 61,645 distinct 1-OP sets of size 3 in average.

\paragraph{Convergence}
Asymptotically, when the number of gateways tends to infinity and the policy spreading is constant, it is clear that the sizes of the 1-OP sets increase so that the number of distinct groups tends to the number of prefixes (the probability that the group of a given prefix is unique tends to one). Similarly, when the policy spreading tends to infinity and the number of gateways is fixed, 1-OP sets sizes decreases, and each prefix obtains a group of size two, which implies that the number of distinct groups tends to $\binom{B}{2}$. Interestingly, when both the number of gateways and the policy spreading tend to infinity similarly (\ie, $ps \sim c B$ with a constant $c$), then the probability that the 1-OP set of a prefix has size $s$ converge to a constant. Unfortunately, that implies that the number of distinct 1-OP sets of size two increases, even if there is the same number of prefixes having a 1-OP of size two (this is because $\binom{2}{B}$ increases). Thus, the total number of distinct groups tends to $P$. Fortunately, as we will see in the next section, the number of gateways in practice is very limited, and on the few cases it appears to be high, the number of prefixes directed towards those gateways is only a small fraction of the total number of prefixes.

